OSIS: Efficient One-stage Network for 3D Instance Segmentation

Current 3D instance segmentation models generally use multi-stage methods to extract instance objects, including clustering, feature extraction, and post-processing processes. However, these multi-stage approaches rely on hyperparameter settings and hand-crafted processes, which restrict the inference speed of the model. In this paper, we propose a new 3D point cloud instance segmentation network, named OSIS. OSIS is a one-stage network, which directly segments instances from 3D point cloud data using neural network. To segment instances directly from the network, we propose an instance decoder, which decodes instance features from the network into instance segments. Our proposed OSIS realizes the end-to-end training by bipartite matching, therefore, our network does not require computationally expensive post-processing steps such as non maximum suppression (NMS) and clustering during inference. The results show that our network finally achieves excellent performance in the commonly used indoor scene instance segmentation dataset, and the inference speed of our network is only an average of 138ms per scene, which substantially exceeds the previous fastest method.

==> ref.tex <==
\begin{thebibliography}{10}

\bibitem{Hou20193DSIS3S}
J.~Hou, A.~Dai, and M.~Nie{\ss}ner, ``3d-sis: 3d semantic instance segmentation
  of rgb-d scans,'' {\em 2019 IEEE/CVF Conference on Computer Vision and
  Pattern Recognition (CVPR)}, pp.~4416--4425, 2019.

\bibitem{Yang2019LearningOB}
B.~Yang, J.~Wang, R.~Clark, Q.~Hu, S.~Wang, A.~Markham, and A.~Trigoni,
  ``Learning object bounding boxes for 3d instance segmentation on point
  clouds,'' {\em ArXiv}, vol.~abs/1906.01140, 2019.

\bibitem{Lahoud20193MTML}
J.~Lahoud, B.~Ghanem, M.~Pollefeys, and M.~R. Oswald, ``3d instance
  segmentation via multi-task metric learning,'' {\em 2019 IEEE/CVF
  International Conference on Computer Vision (ICCV)}, pp.~9255--9265, 2019.

\bibitem{Engelmann20203DMPAMA}
F.~Engelmann, M.~Bokeloh, A.~Fathi, B.~Leibe, and M.~Nie{\ss}ner, ``3d-mpa:
  Multi-proposal aggregation for 3d semantic instance segmentation,'' {\em 2020
  IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pp.~9028--9037, 2020.

\bibitem{He2021DyCo3DRI}
T.~He, C.~Shen, and A.~van~den Hengel, ``Dyco3d: Robust instance segmentation
  of 3d point clouds through dynamic convolution,'' {\em 2021 IEEE/CVF
  Conference on Computer Vision and Pattern Recognition (CVPR)}, pp.~354--363,
  2021.

\bibitem{Zhang2019PE}
B.~Zhang and P.~Wonka, ``Point cloud instance segmentation using probabilistic
  embeddings,'' {\em 2021 IEEE/CVF Conference on Computer Vision and Pattern
  Recognition (CVPR)}, pp.~8879--8888, 2019.

\bibitem{Jiang2020PointGroupDP}
L.~Jiang, H.~Zhao, S.~Shi, S.~Liu, C.-W. Fu, and J.~Jia, ``Pointgroup: Dual-set
  point grouping for 3d instance segmentation,'' {\em 2020 IEEE/CVF Conference
  on Computer Vision and Pattern Recognition (CVPR)}, pp.~4866--4875, 2020.

\bibitem{Wang2017SGPNSG}
W.~Wang, R.~Yu, Q.~Huang, and U.~Neumann, ``Sgpn: Similarity group proposal
  network for 3d point cloud instance segmentation,'' {\em 2018 IEEE/CVF
  Conference on Computer Vision and Pattern Recognition}, pp.~2569--2578, 2017.

\bibitem{Wang2019AssociativelySI}
X.~Wang, S.~Liu, X.~Shen, C.~Shen, and J.~Jia, ``Associatively segmenting
  instances and semantics in point clouds,'' {\em 2019 IEEE/CVF Conference on
  Computer Vision and Pattern Recognition (CVPR)}, pp.~4091--4100, 2019.

\bibitem{Schult2022Mask3DF3}Schult, J., Engelmann, F., Hermans, A., Litany, O., Tang, S. \& Leibe, B. Mask3D for 3D Semantic Instance Segmentation. {\em ArXiv}. abs/2210.03105 (2022)

\bibitem{Yi2019GSPNGS}
L.~Yi, W.~Zhao, H.~Wang, M.~Sung, and L.~J. Guibas, ``Gspn: Generative shape
  proposal network for 3d instance segmentation in point cloud,'' {\em 2019
  IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pp.~3942--3951, 2019.

\bibitem{Liu2020LearningGI}
S.-H. Liu, S.~Yu, S.-C. Wu, H.-T. Chen, and T.-L. Liu, ``Learning gaussian
  instance segmentation in point clouds,'' {\em ArXiv}, vol.~abs/2007.09860,
  2020.

\bibitem{Han2020OccuSegO3}
L.~Han, T.~Zheng, L.~Xu, and L.~Fang, ``Occuseg: Occupancy-aware 3d instance
  segmentation,'' {\em 2020 IEEE/CVF Conference on Computer Vision and Pattern
  Recognition (CVPR)}, pp.~2937--2946, 2020.

\bibitem{liang2021instance}
Z.~Liang, Z.~Li, S.~Xu, M.~Tan, and K.~Jia, ``Instance segmentation in 3d
  scenes using semantic superpoint tree networks,'' {\em 2021 IEEE/CVF
  International Conference on Computer Vision (ICCV)}, pp.~2763--2772, 2021.

\bibitem{Chen2021HierarchicalAF}
S.~Chen, J.~Fang, Q.~Zhang, W.~Liu, and X.~Wang, ``Hierarchical aggregation for
  3d instance segmentation,'' {\em 2021 IEEE/CVF International Conference on
  Computer Vision (ICCV)}, pp.~15447--15456, 2021.

\bibitem{Vu2022SoftGroupF3}
T.~Vu, K.~Kim, T.~M. Luu, X.~T. Nguyen, and C.-D. Yoo, ``Softgroup for 3d
  instance segmentation on point clouds,'' {\em 2022 IEEE/CVF Conference on
  Computer Vision and Pattern Recognition (CVPR)}, pp.~2698--2707, 2022.

\bibitem{Wang2021FCOS3DFC}
T.~Wang, X.~Zhu, J.~Pang, and D.~Lin, ``Fcos3d: Fully convolutional one-stage
  monocular 3d object detection,'' {\em 2021 IEEE/CVF International Conference
  on Computer Vision Workshops (ICCVW)}, pp.~913--922, 2021.

\bibitem{Zhang2020H3DNet3O}
Z.~Zhang, B.~Sun, H.~Yang, and Q.-X. Huang, ``H3dnet: 3d object detection using
  hybrid geometric primitives,'' in {\em European Conference on Computer
  Vision}, 2020.

\bibitem{Pang2021SimpleTrackUA}
Z.~Pang, Z.~Li, and N.~Wang, ``Simpletrack: Understanding and rethinking 3d
  multi-object tracking,'' {\em ArXiv}, vol.~abs/2111.09621, 2021.

\bibitem{text2shape}
K.~Chen, C.~B. Choy, M.~Savva, A.~X. Chang, T.~A. Funkhouser, and S.~Savarese,
  ``Text2shape: Generating shapes from natural language by learning joint
  embeddings,'' in {\em Computer Vision - {ACCV} 2018 - 14th Asian Conference
  on Computer Vision, Perth, Australia, December 2-6, 2018, Revised Selected
  Papers, Part {III}}, pp.~100--116, 2018.

\bibitem{Tang2021Part2WordLJ}
C.~Tang, X.~Yang, B.~Wu, Z.~Han, and Y.~Chang, ``Part2word: Learning joint
  embedding of point clouds and text by matching parts to words,'' {\em ArXiv},
  vol.~abs/2107.01872, 2021.

\bibitem{Wu2020SSTNetDM}
X.~Wu, Z.~Xie, Y.~Gao, and Y.~Xiao, ``Sstnet: Detecting manipulated faces
  through spatial, steganalysis and temporal features,'' {\em ICASSP 2020 -
  2020 IEEE International Conference on Acoustics, Speech and Signal Processing
  (ICASSP)}, pp.~2952--2956, 2020.

\bibitem{Chen2019DynamicCA}
Y.~Chen, X.~Dai, M.~Liu, D.~Chen, L.~Yuan, and Z.~Liu, ``Dynamic convolution:
  Attention over convolution kernels,'' {\em 2020 IEEE/CVF Conference on
  Computer Vision and Pattern Recognition (CVPR)}, pp.~11027--11036, 2019.

\bibitem{Yang2019CondConvCP}
B.~Yang, G.~Bender, Q.~V. Le, and J.~Ngiam, ``Condconv: Conditionally
  parameterized convolutions for efficient inference,'' in {\em Neural
  Information Processing Systems}, 2019.

\bibitem{wang2020solov2}
X.~Wang, R.~Zhang, T.~Kong, L.~Li, and C.~Shen, ``Solov2: Dynamic and fast
  instance segmentation,'' {\em Advances in Neural information processing
  systems}, vol.~33, pp.~17721--17732, 2020.

\bibitem{Tian2020ConditionalCF}
Z.~Tian, C.~Shen, and H.~Chen, ``Conditional convolutions for instance
  segmentation,'' in {\em European Conference on Computer Vision}, 2020.

\bibitem{Cheng2022SparseIA}
T.~Cheng, X.~Wang, S.~Chen, W.~Zhang, Q.~Zhang, C.~Huang, Z.~Zhang, and W.~Liu,
  ``Sparse instance activation for real-time instance segmentation,'' {\em 2022
  IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pp.~4423--4432, 2022.

\bibitem{Dong2021SOLQSO}
B.~Dong, F.~Zeng, T.~Wang, X.~Zhang, and Y.~Wei, ``Solq: Segmenting objects by
  learning queries,'' in {\em Neural Information Processing Systems}, 2021.

\bibitem{Cheng2021MaskFormer}
B.~Cheng, A.~G. Schwing, and A.~Kirillov, ``Per-pixel classification is not all
  you need for semantic segmentation,'' in {\em Neural Information Processing
  Systems}, 2021.

\bibitem{Cheng2022Mask2Former}
B.~Cheng, I.~Misra, A.~G. Schwing, A.~Kirillov, and R.~Girdhar,
  ``Masked-attention mask transformer for universal image segmentation,'' {\em
  2022 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pp.~1280--1289, 2022.

\bibitem{Zhang2021KNetTU}
W.~Zhang, J.~Pang, K.~Chen, and C.~C. Loy, ``K-net: Towards unified image
  segmentation,'' in {\em Neural Information Processing Systems}, 2021.

\bibitem{Erhan2013ScalableOD}
D.~Erhan, C.~Szegedy, A.~Toshev, and D.~Anguelov, ``Scalable object detection
  using deep neural networks,'' {\em 2014 IEEE Conference on Computer Vision
  and Pattern Recognition}, pp.~2155--2162, 2013.

\bibitem{Carion2020DETR}
N.~Carion, F.~Massa, G.~Synnaeve, N.~Usunier, A.~Kirillov, and S.~Zagoruyko,
  ``End-to-end object detection with transformers,'' {\em ArXiv},
  vol.~abs/2005.12872, 2020.

\bibitem{sparseconv}
B.~Graham, M.~Engelcke, and L.~van~der Maaten, ``3d semantic segmentation with
  submanifold sparse convolutional networks,'' {\em 2018 IEEE/CVF Conference on
  Computer Vision and Pattern Recognition}, pp.~9224--9232, 2018.

\bibitem{ronneberger2015unet}
O.~Ronneberger, P.~Fischer, and T.~Brox, ``U-net: Convolutional networks for
  biomedical image segmentation,'' in {\em International Conference on Medical
  image computing and computer-assisted intervention}, pp.~234--241, Springer,
  2015.

\bibitem{Fourier}
M.~Tancik, P.~P. Srinivasan, B.~Mildenhall, S.~Fridovich{-}Keil, N.~Raghavan,
  U.~Singhal, R.~Ramamoorthi, J.~T. Barron, and R.~Ng, ``Fourier features let
  networks learn high frequency functions in low dimensional domains,'' in {\em
  NeurIPS}, 2020.

\bibitem{Dai2017ScanNetR3}
A.~Dai, A.~X. Chang, M.~Savva, M.~Halber, T.~A. Funkhouser, and M.~Nie{\ss}ner,
  ``Scannet: Richly-annotated 3d reconstructions of indoor scenes,'' {\em 2017
  IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pp.~2432--2443, 2017.



\bibitem{Liu20223DQueryISAQ}Liu, J., He, T., Yang, H., Su, R., Tian, J., Wu, J., Guo, H., Xu, K. \& Ouyang, W. 3D-QueryIS: A Query-based Framework for 3D Instance Segmentation. {\em ArXiv}. abs/2211.09375 (2022)

\bibitem{PointInst}He, T., Yin, W., Shen, C. \& Hengel, A. PointInst3D: Segmenting 3D Instances by Points. {\em Computer Vision – ECCV 2022}. pp. 286-302 (2022)

\bibitem{spconv2022}
Y.~Yan, ``Spconv: Spatially sparse convolution library,'' 2022.

\end{thebibliography}

